DeciMamba: Exploring the Length Extrapolation Potential of Mamba

Long-range sequence processing poses a significant challenge for Transformers due to their quadratic complexity in input length. A promising alternative is Mamba, which demonstrates high performance and achieves Transformer-level capabilities while requiring substantially fewer computational resources. In this paper we explore the length-generalization capabilities of Mamba, which we find to be relatively limited. Through a series of visualizations and analyses we identify that the limitations arise from a restricted effective receptive field, dictated by the sequence length used during training. To address this constraint, we introduce DeciMamba, a context-extension method specifically designed for Mamba. This mechanism, built on top of a hidden filtering mechanism embedded within the S6 layer, enables the trained model to extrapolate well even without additional training. Empirical experiments over real-world long-range NLP tasks show that DeciMamba can extrapolate to context lengths that are significantly longer than the ones seen during training, while enjoying faster inference.

==> mamba_attn_eq.tex <==
{\scriptsize
\begin{equation} \label{eq:MambaAttn}
\begin{bmatrix}
y_1 \\
y_2\\ 
\vdots \\
y_L \\
\end{bmatrix} 
=
\begin{bmatrix}
    C_1 \bar{B}_1 & 0 & \cdots & 0 \\
    C_2 \bar{A}_2 \bar{B}_1 & C_2 \bar{B}_2 & \cdots & 0 \\
    \vdots & \vdots & \ddots & 0 \\
    C_L \Pi_{k=2}^L \bar{A}_k \bar{B}_{1} \quad & C_L \Pi_{k=3}^L \bar{A}_k \bar{B}_{2} \quad & \cdots \quad & C_L \bar{B}_L
\end{bmatrix}
\begin{bmatrix}
x_1 \\
x_2\\ 
\vdots \\
x_L \\
\end{bmatrix}
\end{equation}
}

